Detection of statistically significant differences between process variants through declarative rules

Services and products are often offered via the execution of processes that vary according to the context, requirements, or customisation needs. The analysis of such process variants can highlight differences in the service outcome or quality, leading to process adjustments and improvement. Research in the area of process mining has provided several methods for process variants analysis. However, very few of those account for a statistical significance analysis of their output. Moreover, those techniques detect differences at the level of process traces, single activities, or performance. In this paper, we aim at describing the distinctive behavioural characteristics between variants expressed in the form of declarative process rules. The contribution to the research area is two-pronged: the use of declarative rules for the explanation of the process variants and the statistical significance analysis of the outcome. We assess the proposed method by comparing its results to the most recent process variants analysis methods. Our results demonstrate not only that declarative rules reveal differences at an unprecedented level of expressiveness, but also that our method outperforms the state of the art in terms of execution time.

==> addon/commands.tex <==
% Inline lists with roman numbers
\newenvironment{iiilist}%
{\begin{inparaenum}[\itshape(i)\upshape]}%
{\end{inparaenum}}

\RequirePackage{pifont}
\def\CircOne {\ding{192}}
\def\CircTwo {\ding{193}}
\def\CircThree {\ding{194}}
\def\CircFour {\ding{195}}
\def\CircFive {\ding{196}}
\def\CircSix {\ding{197}}
\def\CircSeven {\ding{198}}

\newcommand{\hyperurl}[2]{\href{#1}{\ttfamily #2}}

\newcommand{\grayrow}{\rowcolor{gray!20}} % Requires the colortbl package

%% Check- and cross-marks
\def\GoodExampleMark{\checkmark}
\def\BadExampleMark{$\times$}

\def\dblprime{\ensuremath{^{\prime\prime}\mkern-1.2mu}}
\def\triprime{\ensuremath{^{\prime\prime\prime}\mkern-1.2mu}}
\def\qdrprime{\ensuremath{^{\prime\prime\prime\prime}\mkern-1.2mu}}


==> sections/declare.tex <==
\begin{comment}
%I think we should introduce here a bit of process mining and its basic concepts (log, events, etc), to contextualise declare and this paper. No need for fancy definitions (we can postpone those to the approach section).
A declarative process specification represents the behaviour of a process by means of \emph{constraints}, i.e., temporal rules that specify the conditions under which activities may, must, or cannot be executed.
In this paper we focus on {\Declare}, one of the most well-established declarative process modeling languages to date~\cite{Aalst.etal/CSRD09:DeclarativeWFsBalancing}.

%
{\Declare} provides a standard library of templates (\emph{repertoire} \cite{Polyvyanyy.etal/FAOC2016:ExpressivePowerBehavioralProfiles,DiCiccio.etal/IS2017:ResolvingInconsistenciesRedundanciesDeclare}), i.e., constraints parametrized over activities.
Examples of {\Declare} constraints are
%\begin{iiilist}
%	\item \Resp{\taska}{\taskb},
%	\item \ChaPrec{\taska}{\taskc}, and
%	\item \NotSucc{\taskb}{\taskc}
%\end{iiilist}
\Resp{\taska}{\taskb}
and
\Init{\taskc}.
%
The former constraint applies the {\RespTmp} template on tasks {\taska} and {\taskb}, % (target), 
and states that if {\taska} occurs then {\taskb} must occur later on within the same trace.
In this case, {\taska} is named \emph{activation}, because it is mentioned in the ``if'' clause, thus triggering the constraint, whereas {\taskb} is named \emph{target}, as it is in the consequent clause~\cite{DiCiccio.etal/IS2017:ResolvingInconsistenciesRedundanciesDeclare}.
\Init{\taskc} asserts that every trace must begin with {\taskc}.

Declarative process mining tools can measure to what degree constraints hold true in a given event log~\cite{DBLP:conf/cidm/MaggiMA11}.
To that end, diverse measures have been introduced~\cite{Cecconi2020ATemporal}.
Among them, we consider \emph{confidence} in this context.
Its value ranges from \num{0} to \num{1}.
Let us consider the following example event log:
\todo[inline]{Insert example here. Maybe from an event log we actually use?}
%$\EvtLog = \lbrace {\StrTrc_{1}^{4}}, {\StrTrc_{2}^{1}}, {\StrTrc_{3}^{2}} \rbrace$,
%having
%${\StrTrc_{1}} =
%\Task{baabc}  $,
%${\StrTrc_{2}} =
%\Task{bcc} $, and
%${\StrTrc_{3}} =
%\Task{bcba} $.
%The size of the log is $4+1+2=7$.
%The activations of \Resp{\taska}{\taskb} that satisfy the constraint amount to \num{8} because two {\taska}'s occur in ${\StrTrc_{1}}$ that are eventually followed by an occurrence of {\taskb}, and ${\StrTrc_{1}}$ has multiplicity \num{4} in the event log. The total amount of the constraint's activations in $L$ is \num{10} (see the violating occurrence of {\taska} in ${\StrTrc_{3}}$). The support thus is \num{0.8}.
%By the same line of reasoning, the support of \ChaPrec{\taskb}{\taskc} is $\frac{7}{8}=\num{0.875}$ (notice that in ${\StrTrc_{2}}$ only one of the two occurrences of {\taskc} satisfies the constraint).
%To take into account the frequency with which constraints are triggered, confidence scales support by the ratio of traces in which the activation occurs at least once.
%Therefore, the confidence of \Resp{\taska}{\taskb} is $\num{0.8} \times \frac{6}{7} \approx \num{0.69}$ because {\taska} does not occur in ${\StrTrc_{2}}$. As $\taskb$ occurs in all traces, the confidence of \ChaPrec{\taskb}{\taskc} is \num{0.875}.
\end{comment}
\begin{comment}
From event log $\EvtLog$, it can be inferred that \Resp{\taska}{\taskc} holds true, because in all traces, if {\taska} occurs, eventually {\taskc} occurs too.
On the contrary, \Prec{\taskc}{\taska} is not verified in any trace, as {\taska} is never preceded by {\taskc}. Therefore, the discovered specification should not include \Prec{\taskc}{\taska}.
A degree of uncertainty on whether constraints should be included or not, emerges with constraints that are only partially verified in the event log.
One such example is \Resp{\taska}{\taskb}, because the second occurrence of {\taska} in $\StrTrc_{6}$ is not followed by any {\taskb}, thus violating the constraint.

Measures have been introduced to indicate the level of reliability and relevance of constraints discovered from event logs, originally introduced in the field of association rule mining %~\cite{Adamo/2001:Dataminingassociationrules} 
and adapted to the declarative process discovery context~\cite{Maggi.etal/CIDM2011:UserGuidedDiscovery,DBLP:journals/tmis/CiccioM15}.
For the purpose of this paper, we consider among them
\emph{support} and \emph{confidence}.
Support is a normalized measure quantifying how often the constraint is verified.
Confidence scales the support by the proportion of traces in which the constraint was activated.
\end{comment}
\begin{comment}
In this paper, we consider five of the most commonly occurring templates~\cite{DBLP:conf/icse/DwyerAC99}, depicted in \autoref{tab:declare:explained},
focusing in particular on the ones that are topmost in the subsumption hierarchy of {\Declare} constraints~\cite{DiCiccio.etal/IS2017:ResolvingInconsistenciesRedundanciesDeclare}.
\emph{Existence} constraints are \emph{unary} constraints, i.e., predicating on single tasks. For instance, {\Ini{\taska}} and {\End{\taskb}} establish that all process instances must begin with activity {\taska} and terminate with {\taskb}, respectively.
\emph{Relation} constraints are \emph{binary} and relate the execution of an activity to the occurrence of another one in the same instance (i.e., in one particular execution of the process).
For example, {\Resp{\taska}{\taskb}} requires that if {\taska} is carried out, then {\taskb} must be eventually performed.
{\Prec{\taska}{\taskb}} imposes that {\taskb} cannot be executed if {\taska} has not occurred earlier in the process instance.
{\Succ{\taska}{\taskb}} is a so called \emph{mutual relation} constraint that expresses the joint conditions of {\RespTmp} and {\PrecTmp} over {\taska} and {\taskb}.
Aside from these five templates, we also consider their negative counterparts. For instance,
{\NotSucc{\taska}{\taskb}} is a \emph{negative relation} constraint which states that if {\taska} is executed, then {\taskb} cannot be carried out any longer.
\end{comment}

==> tables/bpic13-output.tex <==
\begin{tabular}{l|l}
    

    & \textbf{Statistically significant differences (\textit{Variant A}: $\mathrm{Company} = \mathrm{A}_{2}$; \textit{Variant B}: $\mathrm{Company} = \mathrm{C}$)} \\\hline
	
	1 & In \textit{Variant A}, it is 10.1\% more likely than \textit{Variant B} that if \taskize{Completed} occurs, also \taskize{Queued} occurs.\\\hline
    2 & In \textit{Variant A}, it is 10.0\% more likely than \textit{Variant B} that if \taskize{Accepted} occurs, also \taskize{Queued} occurs.\\\hline
	3 & In \textit{Variant A}, it is 10.0\% more likely than \textit{Variant B} that \taskize{Queued} occurs in a process instance.\\\hline
    4 & In \textit{Variant A}, it is 9.4\% more likely than \textit{Variant B} that \taskize{Queued} may occur at most once in a process instance.\\\hline
    
\end{tabular}


==> tables/rtfmp-output.tex <==
\begin{tabular}{r|l}
    

    & \textbf{Statistically significant differences (\textit{Variant A}: $\mathrm{Fine} \geq 50$; \textit{Variant B}: $\mathrm{Fine} < 50$)} \\\hline
	
	1 & In \textit{Variant A}, it is 24.8\% more likely than \textit{Variant B} that if \taskize{Payment} occurs, also \taskize{Send Fine} occurs. \\\hline
	2 & In \textit{Variant A}, it is 19.6\% more likely than \textit{Variant B} that if \taskize{Payment} occurs, also \taskize{Add penalty} occurs. \\\hline
    3 & In \textit{Variant A}, it is 19.6\% more likely than \textit{Variant B} that if \taskize{Payment} occurs, also \taskize{Insert Fine Notification} occurs. \\\hline
    4 & In \textit{Variant A}, it is 19.4\% more likely than \textit{Variant B} that \taskize{Add penalty} occurs in a process instance. \\\hline
    5 & In \textit{Variant A}, it is 19.4\% more likely than \textit{Variant B} that \taskize{Insert Fine Notification} occurs in a process instance. \\\hline
    6 & In \textit{Variant A}, it is 19.4\% more likely than \textit{Variant B} that if \taskize{Create Fine} occurs, \taskize{Add penalty} will occur\\ & afterwards without any other occurrence of \taskize{Create Fine} in between. \\\hline
    7 & In \textit{Variant A}, it is 19.4\% more likely than \textit{Variant B} that if \taskize{Create Fine} occurs, \taskize{Insert Fine Notification} will occur\\ & afterwards without any other occurrence of \taskize{Create Fine} in between. \\\hline
    8 & In \textit{Variant A}, it is 19.2\% more likely than \textit{Variant B} that \taskize{Send Fine} occurs in a process instance. \\\hline
    9 & In \textit{Variant A}, it is 19.2\% more likely than \textit{Variant B} that if \taskize{Create Fine} occurs, \taskize{Send Fine} will occur\\ & afterwards without any other occurrence of \taskize{Create Fine} in between. \\\hline
    10 & In \textit{Variant A}, it is 14.5\% more likely than \textit{Variant B} that \taskize{Send for Credit Collection} occurs in a process instance. \\\hline
    11 & In \textit{Variant A}, it is 14.5\% more likely than \textit{Variant B} that if \taskize{Create Fine} occurs, \taskize{Send for Credit Collection} will occur\\ & afterwards without any other occurrence of \taskize{Create Fine} in between. \\\hline
    
\end{tabular}


==> tables/time.tex <==
\begin{table}
\vspace{-1.5\baselineskip}
	\centering
	{\scriptsize{
	\def\arraystretch{1.30} %set distance between rows
\setlength{\tabcolsep}{5pt} %set distance between columns
    \begin{tabular}{l|l|l|l}
    
    \textbf{Logs} 
    & \textbf{DRVA} 
    & \textbf{MFVA} 
    & \textbf{PSEVA} \\\hline
	
	BPIC13 &  \textbf{4.9} & 31.3 & 81.8\\\hline
    BPIC15 &   \textbf{326.7} & 4901.3 & t/o \\\hline
    RTFMP & 38.1 & 1152.9 & \textbf{21.7}\\\hline
    SEPSIS &  \textbf{4.6} & 175.2 & 5.1\\\hline
    
	\end{tabular}
  	\caption{\scriptsize{Execution times (in seconds)}}\label{tab:bpi15}
	}}
\vspace{-2.5\baselineskip}
\end{table}
